How Far Can the Gemma 4 Speech Encoder Go Without Changing Its Weights? Saudi and Gulf Arabic Speech Recognition with a Frozen and an Adapter-Augmented Encoder

We study the 305M-parameter audio encoder shared by Gemma 4 and EmbeddingGemma 2 (bit-identical to that of Gemma 4 E2B except for the final audio-embedding projection) for Saudi and Gulf Arabic speech recognition, without changing any of its pretrained weights; the adapters of our adapted system are additive and kept separate. A frozen system trains only a 22.6M-parameter CTC reader over a learned mix of four intermediate encoder layers and the encoder output; an adapted system adds 3.1M low-rank adapter parameters, a 41.5M-parameter hybrid CTC/attention reader and joint decoding with a sub-word language model. Against Cohere Transcribe Arabic (2.07B parameters), re-run on identical audio, the frozen system trails in word error rate (WER) but is not significantly different in character error rate (CER) on five of six human-labelled conditions, while running 3.4 times faster on CPU with greedy decoding. The adapted system is not significantly different in WER on a public Saudi customer-service call (19.20% against 19.27%) and on clean Emirati speech, is significantly better on telephone-coded Emirati speech, has a significantly lower CER on all six conditions of these sets, and beats a 0.6B recogniser fine-tuned on SADA in WER on all six; it still trails Cohere in WER on long-form Saudi speech. On a blind, human-corrected public call-centre sample it ranks 4 of 15 systems, behind three commercial APIs (significantly only one) and ahead of the other self-hostable systems by point estimate. An optimised joint decoder runs it at 139 times real time on one GPU. We also find, on our data, that references made by correcting machine drafts favour the drafting system. Code and public-set results are released.

==> tables/numbers.tex <==
\makeatletter
\expandafter\def\csname r@ad.casablanca_uae.clean16k.ctclm.cer\endcsname{20.77}
\expandafter\def\csname r@ad.casablanca_uae.clean16k.ctclm.wer\endcsname{50.66}
\expandafter\def\csname r@ad.casablanca_uae.clean16k.greedy.cer\endcsname{20.92}
\expandafter\def\csname r@ad.casablanca_uae.clean16k.greedy.wer\endcsname{56.37}
\expandafter\def\csname r@ad.casablanca_uae.clean16k.jointlm.cer\endcsname{14.89}
\expandafter\def\csname r@ad.casablanca_uae.clean16k.jointlm.wer\endcsname{46.98}
\expandafter\def\csname r@ad.casablanca_uae.tel8k.ctclm.cer\endcsname{23.53}
\expandafter\def\csname r@ad.casablanca_uae.tel8k.ctclm.wer\endcsname{53.50}
\expandafter\def\csname r@ad.casablanca_uae.tel8k.greedy.cer\endcsname{23.80}
\expandafter\def\csname r@ad.casablanca_uae.tel8k.greedy.wer\endcsname{59.81}
\expandafter\def\csname r@ad.casablanca_uae.tel8k.jointlm.cer\endcsname{17.40}
\expandafter\def\csname r@ad.casablanca_uae.tel8k.jointlm.wer\endcsname{50.01}
\expandafter\def\csname r@ad.ctc_alpha\endcsname{0.30}
\expandafter\def\csname r@ad.ctc_beta\endcsname{1.50}
\expandafter\def\csname r@ad.gold.ctclm.cer\endcsname{24.91}
\expandafter\def\csname r@ad.gold.ctclm.wer\endcsname{42.63}
\expandafter\def\csname r@ad.gold.greedy.cer\endcsname{26.14}
\expandafter\def\csname r@ad.gold.greedy.wer\endcsname{50.43}
\expandafter\def\csname r@ad.gold.jointlm.cer\endcsname{22.47}
\expandafter\def\csname r@ad.gold.jointlm.wer\endcsname{42.91}
\expandafter\def\csname r@ad.lenbonus\endcsname{1.00}
\expandafter\def\csname r@ad.lmw\endcsname{0.15}
\expandafter\def\csname r@ad.nb16.casablanca_uae.clean16k.oracle\endcsname{35.63}
\expandafter\def\csname r@ad.nb16.casablanca_uae.tel8k.oracle\endcsname{38.83}
\expandafter\def\csname r@ad.nb16.gold.oracle\endcsname{40.21}
\expandafter\def\csname r@ad.nb16.nexdata_cs_sample.clean16k.oracle\endcsname{13.06}
\expandafter\def\csname r@ad.nb16.nexdata_cs_sample.tel8k.oracle\endcsname{13.84}
\expandafter\def\csname r@ad.nexdata_cs_sample.clean16k.ctclm.cer\endcsname{10.02}
\expandafter\def\csname r@ad.nexdata_cs_sample.clean16k.ctclm.wer\endcsname{20.86}
\expandafter\def\csname r@ad.nexdata_cs_sample.clean16k.greedy.cer\endcsname{11.75}
\expandafter\def\csname r@ad.nexdata_cs_sample.clean16k.greedy.wer\endcsname{27.81}
\expandafter\def\csname r@ad.nexdata_cs_sample.clean16k.jointlm.cer\endcsname{7.77}
\expandafter\def\csname r@ad.nexdata_cs_sample.clean16k.jointlm.wer\endcsname{19.20}
\expandafter\def\csname r@ad.nexdata_cs_sample.tel8k.ctclm.cer\endcsname{10.58}
\expandafter\def\csname r@ad.nexdata_cs_sample.tel8k.ctclm.wer\endcsname{22.61}
\expandafter\def\csname r@ad.nexdata_cs_sample.tel8k.greedy.cer\endcsname{12.23}
\expandafter\def\csname r@ad.nexdata_cs_sample.tel8k.greedy.wer\endcsname{30.24}
\expandafter\def\csname r@ad.nexdata_cs_sample.tel8k.jointlm.cer\endcsname{8.39}
\expandafter\def\csname r@ad.nexdata_cs_sample.tel8k.jointlm.wer\endcsname{21.02}
\expandafter\def\csname r@ad.sada.clean16k.ctclm.cer\endcsname{21.31}
\expandafter\def\csname r@ad.sada.clean16k.ctclm.wer\endcsname{40.38}
\expandafter\def\csname r@ad.sada.clean16k.greedy.cer\endcsname{23.09}
\expandafter\def\csname r@ad.sada.clean16k.greedy.wer\endcsname{48.47}
\expandafter\def\csname r@ad.sada.tel8k.ctclm.cer\endcsname{23.34}
\expandafter\def\csname r@ad.sada.tel8k.ctclm.wer\endcsname{42.51}
\expandafter\def\csname r@ad.sada.tel8k.greedy.cer\endcsname{25.10}
\expandafter\def\csname r@ad.sada.tel8k.greedy.wer\endcsname{51.20}
\expandafter\def\csname r@ad.sauditalk_longform.clean16k.ctclm.cer\endcsname{29.78}
\expandafter\def\csname r@ad.sauditalk_longform.clean16k.ctclm.wer\endcsname{60.29}
\expandafter\def\csname r@ad.sauditalk_longform.clean16k.greedy.cer\endcsname{29.94}
\expandafter\def\csname r@ad.sauditalk_longform.clean16k.greedy.wer\endcsname{64.68}
\expandafter\def\csname r@ad.sauditalk_longform.clean16k.jointlm.cer\endcsname{25.58}
\expandafter\def\csname r@ad.sauditalk_longform.clean16k.jointlm.wer\endcsname{58.79}
\expandafter\def\csname r@ad.sauditalk_longform.tel8k.jointlm.cer\endcsname{26.65}
\expandafter\def\csname r@ad.sauditalk_longform.tel8k.jointlm.wer\endcsname{60.45}
\expandafter\def\csname r@ad.val.lm1\endcsname{29.72}
\expandafter\def\csname r@ad.val.lm2\endcsname{30.05}
\expandafter\def\csname r@api.chirp3.clean16k.cer\endcsname{9.78}
\expandafter\def\csname r@api.chirp3.clean16k.wer\endcsname{26.50}
\expandafter\def\csname r@api.chirp3.d\endcsname{3.39}
\expandafter\def\csname r@api.chirp3.d.hi\endcsname{8.17}
\expandafter\def\csname r@api.chirp3.d.lo\endcsname{-1.48}
\expandafter\def\csname r@api.chirp3.d.n\endcsname{61}
\expandafter\def\csname r@api.chirp3.tel8k.cer\endcsname{10.12}
\expandafter\def\csname r@api.chirp3.tel8k.wer\endcsname{25.70}
\expandafter\def\csname r@api.cohere.clean16k.cer\endcsname{12.11}
\expandafter\def\csname r@api.cohere.clean16k.wer\endcsname{35.06}
\expandafter\def\csname r@api.cohere.d\endcsname{-5.47}
\expandafter\def\csname r@api.cohere.d.hi\endcsname{1.69}
\expandafter\def\csname r@api.cohere.d.lo\endcsname{-12.45}
\expandafter\def\csname r@api.cohere.d.n\endcsname{31}
\expandafter\def\csname r@api.cohere.tel8k.cer\endcsname{14.63}
\expandafter\def\csname r@api.cohere.tel8k.wer\endcsname{33.07}
\expandafter\def\csname r@api.gemini35transcribe.clean16k.cer\endcsname{13.05}
\expandafter\def\csname r@api.gemini35transcribe.clean16k.wer\endcsname{31.33}
\expandafter\def\csname r@api.gemini35transcribe.d\endcsname{-1.44}
\expandafter\def\csname r@api.gemini35transcribe.d.hi\endcsname{4.66}
\expandafter\def\csname r@api.gemini35transcribe.d.lo\endcsname{-8.09}
\expandafter\def\csname r@api.gemini35transcribe.d.n\endcsname{61}
\expandafter\def\csname r@api.gemini35transcribe.tel8k.cer\endcsname{11.62}
\expandafter\def\csname r@api.gemini35transcribe.tel8k.wer\endcsname{29.73}
\expandafter\def\csname r@api.gpt4otranscribe.clean16k.cer\endcsname{27.63}
\expandafter\def\csname r@api.gpt4otranscribe.clean16k.wer\endcsname{38.65}
\expandafter\def\csname r@api.gpt4otranscribe.d\endcsname{-8.76}
\expandafter\def\csname r@api.gpt4otranscribe.d.hi\endcsname{-1.83}
\expandafter\def\csname r@api.gpt4otranscribe.d.lo\endcsname{-15.98}
\expandafter\def\csname r@api.gpt4otranscribe.d.n\endcsname{61}
\expandafter\def\csname r@api.gpt4otranscribe.tel8k.cer\endcsname{30.54}
\expandafter\def\csname r@api.gpt4otranscribe.tel8k.wer\endcsname{44.83}
\expandafter\def\csname r@api.gpttranscribe.clean16k.cer\endcsname{8.14}
\expandafter\def\csname r@api.gpttranscribe.clean16k.wer\endcsname{18.84}
\expandafter\def\csname r@api.gpttranscribe.d\endcsname{11.05}
\expandafter\def\csname r@api.gpttranscribe.d.hi\endcsname{16.17}
\expandafter\def\csname r@api.gpttranscribe.d.lo\endcsname{6.14}
\expandafter\def\csname r@api.gpttranscribe.d.n\endcsname{61}
\expandafter\def\csname r@api.gpttranscribe.tel8k.cer\endcsname{9.13}
\expandafter\def\csname r@api.gpttranscribe.tel8k.wer\endcsname{19.21}
\expandafter\def\csname r@api.grokstt10.clean16k.cer\endcsname{17.12}
\expandafter\def\csname r@api.grokstt10.clean16k.wer\endcsname{31.23}
\expandafter\def\csname r@api.grokstt10.d\endcsname{-1.34}
\expandafter\def\csname r@api.grokstt10.d.hi\endcsname{4.94}
\expandafter\def\csname r@api.grokstt10.d.lo\endcsname{-8.10}
\expandafter\def\csname r@api.grokstt10.d.n\endcsname{61}
\expandafter\def\csname r@api.grokstt10.tel8k.cer\endcsname{14.25}
\expandafter\def\csname r@api.grokstt10.tel8k.wer\endcsname{31.94}
\expandafter\def\csname r@api.maitranscribe2.clean16k.cer\endcsname{9.12}
\expandafter\def\csname r@api.maitranscribe2.clean16k.wer\endcsname{27.28}
\expandafter\def\csname r@api.maitranscribe2.d\endcsname{2.61}
\expandafter\def\csname r@api.maitranscribe2.d.hi\endcsname{6.63}
\expandafter\def\csname r@api.maitranscribe2.d.lo\endcsname{-1.88}
\expandafter\def\csname r@api.maitranscribe2.d.n\endcsname{61}
\expandafter\def\csname r@api.maitranscribe2.tel8k.cer\endcsname{9.11}
\expandafter\def\csname r@api.maitranscribe2.tel8k.wer\endcsname{24.32}
\expandafter\def\csname r@api.n_systems\endcsname{15}
\expandafter\def\csname r@api.nova3.clean16k.cer\endcsname{13.45}
\expandafter\def\csname r@api.nova3.clean16k.wer\endcsname{36.03}
\expandafter\def\csname r@api.nova3.d\endcsname{-6.14}
\expandafter\def\csname r@api.nova3.d.hi\endcsname{-0.14}
\expandafter\def\csname r@api.nova3.d.lo\endcsname{-12.61}
\expandafter\def\csname r@api.nova3.d.n\endcsname{61}
\expandafter\def\csname r@api.nova3.tel8k.cer\endcsname{16.22}
\expandafter\def\csname r@api.nova3.tel8k.wer\endcsname{36.97}
\expandafter\def\csname r@api.rank_ours\endcsname{4}
\expandafter\def\csname r@api.scribev2.clean16k.cer\endcsname{15.02}
\expandafter\def\csname r@api.scribev2.clean16k.wer\endcsname{39.71}
\expandafter\def\csname r@api.scribev2.d\endcsname{-9.50}
\expandafter\def\csname r@api.scribev2.d.hi\endcsname{0.25}
\expandafter\def\csname r@api.scribev2.d.lo\endcsname{-20.10}
\expandafter\def\csname r@api.scribev2.d.n\endcsname{30}
\expandafter\def\csname r@api.scribev2.tel8k.cer\endcsname{17.39}
\expandafter\def\csname r@api.scribev2.tel8k.wer\endcsname{39.38}
\expandafter\def\csname r@api.transcribe1pro.clean16k.cer\endcsname{21.11}
\expandafter\def\csname r@api.transcribe1pro.clean16k.wer\endcsname{39.50}
\expandafter\def\csname r@api.transcribe1pro.d\endcsname{-9.61}
\expandafter\def\csname r@api.transcribe1pro.d.hi\endcsname{-0.91}
\expandafter\def\csname r@api.transcribe1pro.d.lo\endcsname{-19.27}
\expandafter\def\csname r@api.transcribe1pro.d.n\endcsname{61}
\expandafter\def\csname r@api.transcribe1pro.tel8k.cer\endcsname{21.09}
\expandafter\def\csname r@api.transcribe1pro.tel8k.wer\endcsname{38.61}
\expandafter\def\csname r@api.universal35pro.clean16k.cer\endcsname{12.83}
\expandafter\def\csname r@api.universal35pro.clean16k.wer\endcsname{32.15}
\expandafter\def\csname r@api.universal35pro.d\endcsname{-2.26}
\expandafter\def\csname r@api.universal35pro.d.hi\endcsname{4.17}
\expandafter\def\csname r@api.universal35pro.d.lo\endcsname{-9.31}
\expandafter\def\csname r@api.universal35pro.d.n\endcsname{61}
\expandafter\def\csname r@api.universal35pro.tel8k.cer\endcsname{13.89}
\expandafter\def\csname r@api.universal35pro.tel8k.wer\endcsname{32.80}
\expandafter\def\csname r@api.v5db16.clean16k.cer\endcsname{11.30}
\expandafter\def\csname r@api.v5db16.clean16k.wer\endcsname{29.89}
\expandafter\def\csname r@api.v5db16.tel8k.cer\endcsname{11.92}
\expandafter\def\csname r@api.v5db16.tel8k.wer\endcsname{31.51}
\expandafter\def\csname r@api.voxtralminitranscribe.clean16k.cer\endcsname{16.64}
\expandafter\def\csname r@api.voxtralminitranscribe.clean16k.wer\endcsname{38.29}
\expandafter\def\csname r@api.voxtralminitranscribe.d\endcsname{-8.40}
\expandafter\def\csname r@api.voxtralminitranscribe.d.hi\endcsname{-2.17}
\expandafter\def\csname r@api.voxtralminitranscribe.d.lo\endcsname{-15.54}
\expandafter\def\csname r@api.voxtralminitranscribe.d.n\endcsname{61}
\expandafter\def\csname r@api.voxtralminitranscribe.tel8k.cer\endcsname{17.91}
\expandafter\def\csname r@api.voxtralminitranscribe.tel8k.wer\endcsname{39.16}
\expandafter\def\csname r@api.voxtralsmall24b2507stt.clean16k.cer\endcsname{16.71}
\expandafter\def\csname r@api.voxtralsmall24b2507stt.clean16k.wer\endcsname{39.74}
\expandafter\def\csname r@api.voxtralsmall24b2507stt.d\endcsname{-9.85}
\expandafter\def\csname r@api.voxtralsmall24b2507stt.d.hi\endcsname{-2.23}
\expandafter\def\csname r@api.voxtralsmall24b2507stt.d.lo\endcsname{-18.27}
\expandafter\def\csname r@api.voxtralsmall24b2507stt.d.n\endcsname{61}
\expandafter\def\csname r@api.voxtralsmall24b2507stt.tel8k.cer\endcsname{20.53}
\expandafter\def\csname r@api.voxtralsmall24b2507stt.tel8k.wer\endcsname{44.86}
\expandafter\def\csname r@api.whisperlargev3.clean16k.cer\endcsname{22.84}
\expandafter\def\csname r@api.whisperlargev3.clean16k.wer\endcsname{44.35}
\expandafter\def\csname r@api.whisperlargev3.d\endcsname{-14.46}
\expandafter\def\csname r@api.whisperlargev3.d.hi\endcsname{-7.08}
\expandafter\def\csname r@api.whisperlargev3.d.lo\endcsname{-22.21}
\expandafter\def\csname r@api.whisperlargev3.d.n\endcsname{61}
\expandafter\def\csname r@api.whisperlargev3.tel8k.cer\endcsname{22.57}
\expandafter\def\csname r@api.whisperlargev3.tel8k.wer\endcsname{46.74}
\expandafter\def\csname r@best.run\endcsname{v3_tel}
\expandafter\def\csname r@boot.casablanca_uae.clean16k.cer\endcsname{0.91}
\expandafter\def\csname r@boot.casablanca_uae.clean16k.cer.hi\endcsname{2.30}
\expandafter\def\csname r@boot.casablanca_uae.clean16k.cer.lo\endcsname{-0.52}
\expandafter\def\csname r@boot.casablanca_uae.clean16k.wer\endcsname{6.28}
\expandafter\def\csname r@boot.casablanca_uae.clean16k.wer.hi\endcsname{8.05}
\expandafter\def\csname r@boot.casablanca_uae.clean16k.wer.lo\endcsname{4.52}
\expandafter\def\csname r@boot.casablanca_uae.tel8k.cer\endcsname{1.00}
\expandafter\def\csname r@boot.casablanca_uae.tel8k.cer.hi\endcsname{2.59}
\expandafter\def\csname r@boot.casablanca_uae.tel8k.cer.lo\endcsname{-0.60}
\expandafter\def\csname r@boot.casablanca_uae.tel8k.wer\endcsname{5.67}
\expandafter\def\csname r@boot.casablanca_uae.tel8k.wer.hi\endcsname{7.57}
\expandafter\def\csname r@boot.casablanca_uae.tel8k.wer.lo\endcsname{3.74}
\expandafter\def\csname r@boot.nexdata_cs_sample.clean16k.cer\endcsname{1.85}
\expandafter\def\csname r@boot.nexdata_cs_sample.clean16k.cer.hi\endcsname{4.00}
\expandafter\def\csname r@boot.nexdata_cs_sample.clean16k.cer.lo\endcsname{-0.44}
\expandafter\def\csname r@boot.nexdata_cs_sample.clean16k.wer\endcsname{10.35}
\expandafter\def\csname r@boot.nexdata_cs_sample.clean16k.wer.hi\endcsname{13.50}
\expandafter\def\csname r@boot.nexdata_cs_sample.clean16k.wer.lo\endcsname{7.16}
\expandafter\def\csname r@boot.nexdata_cs_sample.tel8k.cer\endcsname{1.81}
\expandafter\def\csname r@boot.nexdata_cs_sample.tel8k.cer.hi\endcsname{3.65}
\expandafter\def\csname r@boot.nexdata_cs_sample.tel8k.cer.lo\endcsname{-0.06}
\expandafter\def\csname r@boot.nexdata_cs_sample.tel8k.wer\endcsname{10.10}
\expandafter\def\csname r@boot.nexdata_cs_sample.tel8k.wer.hi\endcsname{12.79}
\expandafter\def\csname r@boot.nexdata_cs_sample.tel8k.wer.lo\endcsname{7.49}
\expandafter\def\csname r@boot.sauditalk_longform.clean16k.cer\endcsname{0.09}
\expandafter\def\csname r@boot.sauditalk_longform.clean16k.cer.hi\endcsname{1.56}
\expandafter\def\csname r@boot.sauditalk_longform.clean16k.cer.lo\endcsname{-1.58}
\expandafter\def\csname r@boot.sauditalk_longform.clean16k.wer\endcsname{8.54}
\expandafter\def\csname r@boot.sauditalk_longform.clean16k.wer.hi\endcsname{10.20}
\expandafter\def\csname r@boot.sauditalk_longform.clean16k.wer.lo\endcsname{6.89}
\expandafter\def\csname r@boot.sauditalk_longform.tel8k.cer\endcsname{2.96}
\expandafter\def\csname r@boot.sauditalk_longform.tel8k.cer.hi\endcsname{3.96}
\expandafter\def\csname r@boot.sauditalk_longform.tel8k.cer.lo\endcsname{1.96}
\expandafter\def\csname r@boot.sauditalk_longform.tel8k.wer\endcsname{10.76}
\expandafter\def\csname r@boot.sauditalk_longform.tel8k.wer.hi\endcsname{12.14}
\expandafter\def\csname r@boot.sauditalk_longform.tel8k.wer.lo\endcsname{9.37}
\expandafter\def\csname r@boot5.casablanca_uae.clean16k.cer\endcsname{-5.47}
\expandafter\def\csname r@boot5.casablanca_uae.clean16k.cer.hi\endcsname{-4.10}
\expandafter\def\csname r@boot5.casablanca_uae.clean16k.cer.lo\endcsname{-6.88}
\expandafter\def\csname r@boot5.casablanca_uae.clean16k.wer\endcsname{-1.37}
\expandafter\def\csname r@boot5.casablanca_uae.clean16k.wer.hi\endcsname{0.43}
\expandafter\def\csname r@boot5.casablanca_uae.clean16k.wer.lo\endcsname{-3.11}
\expandafter\def\csname r@boot5.casablanca_uae.tel8k.cer\endcsname{-6.98}
\expandafter\def\csname r@boot5.casablanca_uae.tel8k.cer.hi\endcsname{-5.40}
\expandafter\def\csname r@boot5.casablanca_uae.tel8k.cer.lo\endcsname{-8.63}
\expandafter\def\csname r@boot5.casablanca_uae.tel8k.wer\endcsname{-3.14}
\expandafter\def\csname r@boot5.casablanca_uae.tel8k.wer.hi\endcsname{-1.32}
\expandafter\def\csname r@boot5.casablanca_uae.tel8k.wer.lo\endcsname{-5.01}
\expandafter\def\csname r@boot5.nexdata_cs_sample.clean16k.cer\endcsname{-2.28}
\expandafter\def\csname r@boot5.nexdata_cs_sample.clean16k.cer.hi\endcsname{-0.21}
\expandafter\def\csname r@boot5.nexdata_cs_sample.clean16k.cer.lo\endcsname{-4.45}
\expandafter\def\csname r@boot5.nexdata_cs_sample.clean16k.wer\endcsname{-0.07}
\expandafter\def\csname r@boot5.nexdata_cs_sample.clean16k.wer.hi\endcsname{3.48}
\expandafter\def\csname r@boot5.nexdata_cs_sample.clean16k.wer.lo\endcsname{-3.90}
\expandafter\def\csname r@boot5.nexdata_cs_sample.tel8k.cer\endcsname{-2.53}
\expandafter\def\csname r@boot5.nexdata_cs_sample.tel8k.cer.hi\endcsname{-0.84}
\expandafter\def\csname r@boot5.nexdata_cs_sample.tel8k.cer.lo\endcsname{-4.23}
\expandafter\def\csname r@boot5.nexdata_cs_sample.tel8k.wer\endcsname{0.49}
\expandafter\def\csname r@boot5.nexdata_cs_sample.tel8k.wer.hi\endcsname{3.46}
\expandafter\def\csname r@boot5.nexdata_cs_sample.tel8k.wer.lo\endcsname{-2.51}
\expandafter\def\csname r@boot5.sauditalk_longform.clean16k.cer\endcsname{-3.93}
\expandafter\def\csname r@boot5.sauditalk_longform.clean16k.cer.hi\endcsname{-2.49}
\expandafter\def\csname r@boot5.sauditalk_longform.clean16k.cer.lo\endcsname{-5.59}
\expandafter\def\csname r@boot5.sauditalk_longform.clean16k.wer\endcsname{2.04}
\expandafter\def\csname r@boot5.sauditalk_longform.clean16k.wer.hi\endcsname{3.41}
\expandafter\def\csname r@boot5.sauditalk_longform.clean16k.wer.lo\endcsname{0.64}
\expandafter\def\csname r@boot5.sauditalk_longform.tel8k.cer\endcsname{-1.76}
\expandafter\def\csname r@boot5.sauditalk_longform.tel8k.cer.hi\endcsname{-0.73}
\expandafter\def\csname r@boot5.sauditalk_longform.tel8k.cer.lo\endcsname{-2.85}
\expandafter\def\csname r@boot5.sauditalk_longform.tel8k.wer\endcsname{4.64}
\expandafter\def\csname r@boot5.sauditalk_longform.tel8k.wer.hi\endcsname{5.86}
\expandafter\def\csname r@boot5.sauditalk_longform.tel8k.wer.lo\endcsname{3.41}
\expandafter\def\csname r@bootn.casablanca_uae.clean16k.cer\endcsname{-2.20}
\expandafter\def\csname r@bootn.casablanca_uae.clean16k.cer.hi\endcsname{-1.50}
\expandafter\def\csname r@bootn.casablanca_uae.clean16k.cer.lo\endcsname{-2.92}
\expandafter\def\csname r@bootn.casablanca_uae.clean16k.wer\endcsname{-6.28}
\expandafter\def\csname r@bootn.casablanca_uae.clean16k.wer.hi\endcsname{-4.88}
\expandafter\def\csname r@bootn.casablanca_uae.clean16k.wer.lo\endcsname{-7.70}
\expandafter\def\csname r@bootn.casablanca_uae.tel8k.cer\endcsname{-2.41}
\expandafter\def\csname r@bootn.casablanca_uae.tel8k.cer.hi\endcsname{-1.63}
\expandafter\def\csname r@bootn.casablanca_uae.tel8k.cer.lo\endcsname{-3.17}
\expandafter\def\csname r@bootn.casablanca_uae.tel8k.wer\endcsname{-6.55}
\expandafter\def\csname r@bootn.casablanca_uae.tel8k.wer.hi\endcsname{-5.13}
\expandafter\def\csname r@bootn.casablanca_uae.tel8k.wer.lo\endcsname{-8.00}
\expandafter\def\csname r@bootn.nexdata_cs_sample.clean16k.cer\endcsname{-0.81}
\expandafter\def\csname r@bootn.nexdata_cs_sample.clean16k.cer.hi\endcsname{0.38}
\expandafter\def\csname r@bootn.nexdata_cs_sample.clean16k.cer.lo\endcsname{-2.05}
\expandafter\def\csname r@bootn.nexdata_cs_sample.clean16k.wer\endcsname{-4.92}
\expandafter\def\csname r@bootn.nexdata_cs_sample.clean16k.wer.hi\endcsname{-1.68}
\expandafter\def\csname r@bootn.nexdata_cs_sample.clean16k.wer.lo\endcsname{-8.25}
\expandafter\def\csname r@bootn.nexdata_cs_sample.tel8k.cer\endcsname{-1.46}
\expandafter\def\csname r@bootn.nexdata_cs_sample.tel8k.cer.hi\endcsname{-0.12}
\expandafter\def\csname r@bootn.nexdata_cs_sample.tel8k.cer.lo\endcsname{-2.88}
\expandafter\def\csname r@bootn.nexdata_cs_sample.tel8k.wer\endcsname{-4.39}
\expandafter\def\csname r@bootn.nexdata_cs_sample.tel8k.wer.hi\endcsname{-1.07}
\expandafter\def\csname r@bootn.nexdata_cs_sample.tel8k.wer.lo\endcsname{-7.81}
\expandafter\def\csname r@bootn.sauditalk_longform.clean16k.cer\endcsname{-0.19}
\expandafter\def\csname r@bootn.sauditalk_longform.clean16k.cer.hi\endcsname{0.23}
\expandafter\def\csname r@bootn.sauditalk_longform.clean16k.cer.lo\endcsname{-0.59}
\expandafter\def\csname r@bootn.sauditalk_longform.clean16k.wer\endcsname{-2.46}
\expandafter\def\csname r@bootn.sauditalk_longform.clean16k.wer.hi\endcsname{-1.59}
\expandafter\def\csname r@bootn.sauditalk_longform.clean16k.wer.lo\endcsname{-3.35}
\expandafter\def\csname r@bootn.sauditalk_longform.tel8k.cer\endcsname{-0.58}
\expandafter\def\csname r@bootn.sauditalk_longform.tel8k.cer.hi\endcsname{-0.15}
\expandafter\def\csname r@bootn.sauditalk_longform.tel8k.cer.lo\endcsname{-1.00}
\expandafter\def\csname r@bootn.sauditalk_longform.tel8k.wer\endcsname{-2.18}
\expandafter\def\csname r@bootn.sauditalk_longform.tel8k.wer.hi\endcsname{-1.33}
\expandafter\def\csname r@bootn.sauditalk_longform.tel8k.wer.lo\endcsname{-3.02}
\expandafter\def\csname r@corpus.casablanca_uae.clean16k.cohere\endcsname{47.52}
\expandafter\def\csname r@corpus.casablanca_uae.clean16k.ours\endcsname{53.53}
\expandafter\def\csname r@corpus.casablanca_uae.tel8k.cohere\endcsname{51.75}
\expandafter\def\csname r@corpus.casablanca_uae.tel8k.ours\endcsname{57.32}
\expandafter\def\csname r@corpus.nexdata_cs_sample.clean16k.cohere\endcsname{20.77}
\expandafter\def\csname r@corpus.nexdata_cs_sample.clean16k.ours\endcsname{30.12}
\expandafter\def\csname r@corpus.nexdata_cs_sample.tel8k.cohere\endcsname{21.87}
\expandafter\def\csname r@corpus.nexdata_cs_sample.tel8k.ours\endcsname{31.91}
\expandafter\def\csname r@corpus.sauditalk_longform.clean16k.cohere\endcsname{52.69}
\expandafter\def\csname r@corpus.sauditalk_longform.clean16k.ours\endcsname{61.35}
\expandafter\def\csname r@corpus.sauditalk_longform.tel8k.cohere\endcsname{51.89}
\expandafter\def\csname r@corpus.sauditalk_longform.tel8k.ours\endcsname{63.07}
\expandafter\def\csname r@corpus5.casablanca_uae.clean16k\endcsname{47.38}
\expandafter\def\csname r@corpus5.casablanca_uae.tel8k\endcsname{50.06}
\expandafter\def\csname r@corpus5.nexdata_cs_sample.clean16k\endcsname{19.81}
\expandafter\def\csname r@corpus5.nexdata_cs_sample.tel8k\endcsname{21.60}
\expandafter\def\csname r@corpus5.sauditalk_longform.clean16k\endcsname{54.34}
\expandafter\def\csname r@corpus5.sauditalk_longform.tel8k\endcsname{56.20}
\expandafter\def\csname r@do.cohere.clean16k.cer\endcsname{14.59}
\expandafter\def\csname r@do.cohere.clean16k.clear.cer\endcsname{14.59}
\expandafter\def\csname r@do.cohere.clean16k.clear.n\endcsname{62}
\expandafter\def\csname r@do.cohere.clean16k.clear.wer\endcsname{34.17}
\expandafter\def\csname r@do.cohere.clean16k.n\endcsname{62}
\expandafter\def\csname r@do.cohere.clean16k.wer\endcsname{34.17}
\expandafter\def\csname r@do.cohere.tel8k.cer\endcsname{14.10}
\expandafter\def\csname r@do.cohere.tel8k.clear.cer\endcsname{14.10}
\expandafter\def\csname r@do.cohere.tel8k.clear.n\endcsname{62}
\expandafter\def\csname r@do.cohere.tel8k.clear.wer\endcsname{30.87}
\expandafter\def\csname r@do.cohere.tel8k.n\endcsname{62}
\expandafter\def\csname r@do.cohere.tel8k.wer\endcsname{30.87}
\expandafter\def\csname r@do.drafted.cohere\endcsname{30}
\expandafter\def\csname r@do.drafted.ours\endcsname{31}
\expandafter\def\csname r@do.drafted.scribe\endcsname{31}
\expandafter\def\csname r@do.fail100.cohere\endcsname{3}
\expandafter\def\csname r@do.fail100.scribe_v2\endcsname{7}
\expandafter\def\csname r@do.fail100.v5d_b16\endcsname{2}
\expandafter\def\csname r@do.median.cohere\endcsname{25.0}
\expandafter\def\csname r@do.median.scribe_v2\endcsname{25.0}
\expandafter\def\csname r@do.median.v5d_b16\endcsname{27.3}
\expandafter\def\csname r@do.minutes\endcsname{8.3}
\expandafter\def\csname r@do.nclips\endcsname{92}
\expandafter\def\csname r@do.nwords\endcsname{854}
\expandafter\def\csname r@do.scribe_v2.clean16k.cer\endcsname{17.16}
\expandafter\def\csname r@do.scribe_v2.clean16k.clear.cer\endcsname{17.16}
\expandafter\def\csname r@do.scribe_v2.clean16k.clear.n\endcsname{61}
\expandafter\def\csname r@do.scribe_v2.clean16k.clear.wer\endcsname{35.32}
\expandafter\def\csname r@do.scribe_v2.clean16k.n\endcsname{61}
\expandafter\def\csname r@do.scribe_v2.clean16k.wer\endcsname{35.32}
\expandafter\def\csname r@do.scribe_v2.tel8k.cer\endcsname{19.30}
\expandafter\def\csname r@do.scribe_v2.tel8k.clear.cer\endcsname{19.30}
\expandafter\def\csname r@do.scribe_v2.tel8k.clear.n\endcsname{61}
\expandafter\def\csname r@do.scribe_v2.tel8k.clear.wer\endcsname{37.00}
\expandafter\def\csname r@do.scribe_v2.tel8k.n\endcsname{61}
\expandafter\def\csname r@do.scribe_v2.tel8k.wer\endcsname{37.00}
\expandafter\def\csname r@do.unchanged.cohere\endcsname{16}
\expandafter\def\csname r@do.unchanged.ours\endcsname{18}
\expandafter\def\csname r@do.unchanged.scribe\endcsname{23}
\expandafter\def\csname r@do.v5d_b16.clean16k.cer\endcsname{11.30}
\expandafter\def\csname r@do.v5d_b16.clean16k.clear.cer\endcsname{11.30}
\expandafter\def\csname r@do.v5d_b16.clean16k.clear.n\endcsname{61}
\expandafter\def\csname r@do.v5d_b16.clean16k.clear.wer\endcsname{29.89}
\expandafter\def\csname r@do.v5d_b16.clean16k.n\endcsname{61}
\expandafter\def\csname r@do.v5d_b16.clean16k.wer\endcsname{29.89}
\expandafter\def\csname r@do.v5d_b16.tel8k.cer\endcsname{11.92}
\expandafter\def\csname r@do.v5d_b16.tel8k.clear.cer\endcsname{11.92}
\expandafter\def\csname r@do.v5d_b16.tel8k.clear.n\endcsname{61}
\expandafter\def\csname r@do.v5d_b16.tel8k.clear.wer\endcsname{31.51}
\expandafter\def\csname r@do.v5d_b16.tel8k.n\endcsname{61}
\expandafter\def\csname r@do.v5d_b16.tel8k.wer\endcsname{31.51}
\expandafter\def\csname r@dob.cohere.clean16k.cer\endcsname{-0.14}
\expandafter\def\csname r@dob.cohere.clean16k.cer.hi\endcsname{3.42}
\expandafter\def\csname r@dob.cohere.clean16k.cer.lo\endcsname{-4.82}
\expandafter\def\csname r@dob.cohere.clean16k.n\endcsname{31}
\expandafter\def\csname r@dob.cohere.clean16k.wer\endcsname{-5.47}
\expandafter\def\csname r@dob.cohere.clean16k.wer.hi\endcsname{1.81}
\expandafter\def\csname r@dob.cohere.clean16k.wer.lo\endcsname{-12.55}
\expandafter\def\csname r@dob.cohere.tel8k.cer\endcsname{-3.36}
\expandafter\def\csname r@dob.cohere.tel8k.cer.hi\endcsname{1.04}
\expandafter\def\csname r@dob.cohere.tel8k.cer.lo\endcsname{-8.47}
\expandafter\def\csname r@dob.cohere.tel8k.n\endcsname{31}
\expandafter\def\csname r@dob.cohere.tel8k.wer\endcsname{-4.22}
\expandafter\def\csname r@dob.cohere.tel8k.wer.hi\endcsname{4.76}
\expandafter\def\csname r@dob.cohere.tel8k.wer.lo\endcsname{-13.84}
\expandafter\def\csname r@dob.scribe_v2.clean16k.cer\endcsname{-4.41}
\expandafter\def\csname r@dob.scribe_v2.clean16k.cer.hi\endcsname{-0.87}
\expandafter\def\csname r@dob.scribe_v2.clean16k.cer.lo\endcsname{-8.58}
\expandafter\def\csname r@dob.scribe_v2.clean16k.n\endcsname{30}
\expandafter\def\csname r@dob.scribe_v2.clean16k.wer\endcsname{-9.50}
\expandafter\def\csname r@dob.scribe_v2.clean16k.wer.hi\endcsname{0.18}
\expandafter\def\csname r@dob.scribe_v2.clean16k.wer.lo\endcsname{-20.30}
\expandafter\def\csname r@dob.scribe_v2.tel8k.cer\endcsname{-4.80}
\expandafter\def\csname r@dob.scribe_v2.tel8k.cer.hi\endcsname{0.44}
\expandafter\def\csname r@dob.scribe_v2.tel8k.cer.lo\endcsname{-11.43}
\expandafter\def\csname r@dob.scribe_v2.tel8k.n\endcsname{30}
\expandafter\def\csname r@dob.scribe_v2.tel8k.wer\endcsname{-5.13}
\expandafter\def\csname r@dob.scribe_v2.tel8k.wer.hi\endcsname{4.37}
\expandafter\def\csname r@dob.scribe_v2.tel8k.wer.lo\endcsname{-16.37}
\expandafter\def\csname r@fast.audio_s\endcsname{827}
\expandafter\def\csname r@fast.batch\endcsname{16}
\expandafter\def\csname r@fast.files\endcsname{198}
\expandafter\def\csname r@fast.gpuh_per_1000h\endcsname{7.2}
\expandafter\def\csname r@fast.p1.cscer\endcsname{8.34}
\expandafter\def\csname r@fast.p1.cswer\endcsname{20.32}
\expandafter\def\csname r@fast.p1.rtfx\endcsname{68}
\expandafter\def\csname r@fast.p2.cscer\endcsname{8.38}
\expandafter\def\csname r@fast.p2.cswer\endcsname{20.48}
\expandafter\def\csname r@fast.p2.rtfx\endcsname{106}
\expandafter\def\csname r@fast.p3.cscer\endcsname{8.38}
\expandafter\def\csname r@fast.p3.cswer\endcsname{20.48}
\expandafter\def\csname r@fast.p3.rtfx\endcsname{133}
\expandafter\def\csname r@fast.p4.cscer\endcsname{8.38}
\expandafter\def\csname r@fast.p4.cswer\endcsname{20.48}
\expandafter\def\csname r@fast.p4.rtfx\endcsname{139}
\expandafter\def\csname r@fast.speedup\endcsname{82}
\expandafter\def\csname r@gold.best.corpus_wer\endcsname{49.14}
\expandafter\def\csname r@gold.better_windows\endcsname{10}
\expandafter\def\csname r@gold.calls\endcsname{63}
\expandafter\def\csname r@gold.cohere.cer\endcsname{19.67}
\expandafter\def\csname r@gold.cohere.corpus_wer\endcsname{40.13}
\expandafter\def\csname r@gold.cohere.numbers.wer\endcsname{38.00}
\expandafter\def\csname r@gold.cohere.speech.wer\endcsname{37.36}
\expandafter\def\csname r@gold.cohere.src.coh.wer\endcsname{43.60}
\expandafter\def\csname r@gold.cohere.src.dg.wer\endcsname{30.88}
\expandafter\def\csname r@gold.cohere.src.edited.wer\endcsname{42.37}
\expandafter\def\csname r@gold.cohere.wer\endcsname{37.62}
\expandafter\def\csname r@gold.diff\endcsname{9.59}
\expandafter\def\csname r@gold.diff.chi\endcsname{12.88}
\expandafter\def\csname r@gold.diff.clo\endcsname{6.68}
\expandafter\def\csname r@gold.diff.hi\endcsname{12.98}
\expandafter\def\csname r@gold.diff.lo\endcsname{6.65}
\expandafter\def\csname r@gold.diffnemo\endcsname{0.49}
\expandafter\def\csname r@gold.diffnemo.chi\endcsname{3.68}
\expandafter\def\csname r@gold.diffnemo.clo\endcsname{-2.49}
\expandafter\def\csname r@gold.diffnemo.hi\endcsname{3.71}
\expandafter\def\csname r@gold.diffnemo.lo\endcsname{-2.58}
\expandafter\def\csname r@gold.firstpass_cloud.cer\endcsname{25.04}
\expandafter\def\csname r@gold.firstpass_cloud.numbers.wer\endcsname{30.95}
\expandafter\def\csname r@gold.firstpass_cloud.speech.wer\endcsname{38.66}
\expandafter\def\csname r@gold.firstpass_cloud.wer\endcsname{35.56}
\expandafter\def\csname r@gold.firstpass_cohere.cer\endcsname{21.30}
\expandafter\def\csname r@gold.firstpass_cohere.numbers.wer\endcsname{34.88}
\expandafter\def\csname r@gold.firstpass_cohere.speech.wer\endcsname{27.35}
\expandafter\def\csname r@gold.firstpass_cohere.wer\endcsname{30.39}
\expandafter\def\csname r@gold.n\endcsname{72}
\expandafter\def\csname r@gold.n.numbers\endcsname{29}
\expandafter\def\csname r@gold.n.speech\endcsname{43}
\expandafter\def\csname r@gold.nemo_base.cer\endcsname{25.83}
\expandafter\def\csname r@gold.nemo_base.numbers.wer\endcsname{51.01}
\expandafter\def\csname r@gold.nemo_base.speech.wer\endcsname{51.54}
\expandafter\def\csname r@gold.nemo_base.wer\endcsname{51.33}
\expandafter\def\csname r@gold.nemo_ft.cer\endcsname{21.47}
\expandafter\def\csname r@gold.nemo_ft.corpus_wer\endcsname{48.33}
\expandafter\def\csname r@gold.nemo_ft.numbers.wer\endcsname{45.67}
\expandafter\def\csname r@gold.nemo_ft.speech.wer\endcsname{47.41}
\expandafter\def\csname r@gold.nemo_ft.src.coh.wer\endcsname{56.16}
\expandafter\def\csname r@gold.nemo_ft.src.dg.wer\endcsname{35.94}
\expandafter\def\csname r@gold.nemo_ft.src.edited.wer\endcsname{54.72}
\expandafter\def\csname r@gold.nemo_ft.wer\endcsname{46.71}
\expandafter\def\csname r@gold.prov.coh.gap\endcsname{14.78}
\expandafter\def\csname r@gold.prov.dg.gap\endcsname{5.40}
\expandafter\def\csname r@gold.prov.edited.gap\endcsname{7.64}
\expandafter\def\csname r@gold.src.n.coh\endcsname{30}
\expandafter\def\csname r@gold.src.n.dg\endcsname{33}
\expandafter\def\csname r@gold.src.n.edited\endcsname{9}
\expandafter\def\csname r@gold.src.n.unchanged\endcsname{63}
\expandafter\def\csname r@gold.v2.greedy.cer\endcsname{27.10}
\expandafter\def\csname r@gold.v2.greedy.numbers.wer\endcsname{60.01}
\expandafter\def\csname r@gold.v2.greedy.speech.wer\endcsname{60.71}
\expandafter\def\csname r@gold.v2.greedy.wer\endcsname{60.43}
\expandafter\def\csname r@gold.v2.lm.cer\endcsname{25.99}
\expandafter\def\csname r@gold.v2.lm.numbers.wer\endcsname{48.63}
\expandafter\def\csname r@gold.v2.lm.speech.wer\endcsname{49.25}
\expandafter\def\csname r@gold.v2.lm.src.coh.wer\endcsname{60.11}
\expandafter\def\csname r@gold.v2.lm.src.dg.wer\endcsname{37.87}
\expandafter\def\csname r@gold.v2.lm.src.edited.wer\endcsname{52.75}
\expandafter\def\csname r@gold.v2.lm.wer\endcsname{49.00}
\expandafter\def\csname r@gold.v3_tel.greedy.cer\endcsname{25.61}
\expandafter\def\csname r@gold.v3_tel.greedy.numbers.wer\endcsname{58.07}
\expandafter\def\csname r@gold.v3_tel.greedy.speech.wer\endcsname{59.11}
\expandafter\def\csname r@gold.v3_tel.greedy.wer\endcsname{58.69}
\expandafter\def\csname r@gold.v3_tel.lm.cer\endcsname{25.32}
\expandafter\def\csname r@gold.v3_tel.lm.corpus_wer\endcsname{49.14}
\expandafter\def\csname r@gold.v3_tel.lm.numbers.wer\endcsname{46.47}
\expandafter\def\csname r@gold.v3_tel.lm.speech.wer\endcsname{47.70}
\expandafter\def\csname r@gold.v3_tel.lm.src.coh.wer\endcsname{58.38}
\expandafter\def\csname r@gold.v3_tel.lm.src.dg.wer\endcsname{36.28}
\expandafter\def\csname r@gold.v3_tel.lm.src.edited.wer\endcsname{50.01}
\expandafter\def\csname r@gold.v3_tel.lm.wer\endcsname{47.20}
\expandafter\def\csname r@gold.v3_wide.greedy.cer\endcsname{25.65}
\expandafter\def\csname r@gold.v3_wide.greedy.numbers.wer\endcsname{58.12}
\expandafter\def\csname r@gold.v3_wide.greedy.speech.wer\endcsname{58.18}
\expandafter\def\csname r@gold.v3_wide.greedy.wer\endcsname{58.15}
\expandafter\def\csname r@gold.v3_wide.lm.cer\endcsname{25.47}
\expandafter\def\csname r@gold.v3_wide.lm.numbers.wer\endcsname{47.41}
\expandafter\def\csname r@gold.v3_wide.lm.speech.wer\endcsname{47.16}
\expandafter\def\csname r@gold.v3_wide.lm.src.coh.wer\endcsname{57.54}
\expandafter\def\csname r@gold.v3_wide.lm.src.dg.wer\endcsname{37.14}
\expandafter\def\csname r@gold.v3_wide.lm.src.edited.wer\endcsname{50.11}
\expandafter\def\csname r@gold.v3_wide.lm.wer\endcsname{47.26}
\expandafter\def\csname r@gold.worse_windows\endcsname{56}
\expandafter\def\csname r@ladder.chars_frozen\endcsname{46.87}
\expandafter\def\csname r@ladder.ffn_lora\endcsname{38.59}
\expandafter\def\csname r@ladder.hybrid\endcsname{40.51}
\expandafter\def\csname r@ladder.hybrid_selfcond\endcsname{40.01}
\expandafter\def\csname r@ladder.subword_frozen\endcsname{57.19}
\expandafter\def\csname r@ladder.subword_lora\endcsname{49.15}
\expandafter\def\csname r@lit.cohere\endcsname{37.47}
\expandafter\def\csname r@lit.nemo_lm\endcsname{44.52}
\expandafter\def\csname r@lit.whisper\endcsname{55.96}
\expandafter\def\csname r@mix.v2.10\endcsname{22.1}
\expandafter\def\csname r@mix.v2.11\endcsname{23.8}
\expandafter\def\csname r@mix.v2.12\endcsname{9.9}
\expandafter\def\csname r@mix.v2.6\endcsname{25.6}
\expandafter\def\csname r@mix.v2.8\endcsname{8.6}
\expandafter\def\csname r@mix.v2.out\endcsname{9.9}
\expandafter\def\csname r@mix.v3_tel.10\endcsname{21.8}
\expandafter\def\csname r@mix.v3_tel.11\endcsname{25.9}
\expandafter\def\csname r@mix.v3_tel.12\endcsname{9.5}
\expandafter\def\csname r@mix.v3_tel.6\endcsname{25.6}
\expandafter\def\csname r@mix.v3_tel.8\endcsname{7.8}
\expandafter\def\csname r@mix.v3_tel.out\endcsname{9.4}
\expandafter\def\csname r@mix.v3_wide.10\endcsname{21.9}
\expandafter\def\csname r@mix.v3_wide.11\endcsname{26.0}
\expandafter\def\csname r@mix.v3_wide.12\endcsname{9.6}
\expandafter\def\csname r@mix.v3_wide.6\endcsname{25.3}
\expandafter\def\csname r@mix.v3_wide.8\endcsname{7.8}
\expandafter\def\csname r@mix.v3_wide.out\endcsname{9.5}
\expandafter\def\csname r@oracle.lm.top1\endcsname{47.63}
\expandafter\def\csname r@oracle.lm.top128\endcsname{45.10}
\expandafter\def\csname r@oracle.lm.top32\endcsname{45.25}
\expandafter\def\csname r@oracle.lm.top8\endcsname{46.03}
\expandafter\def\csname r@oracle.no_lm.top1\endcsname{56.78}
\expandafter\def\csname r@oracle.no_lm.top128\endcsname{54.24}
\expandafter\def\csname r@oracle.no_lm.top32\endcsname{54.70}
\expandafter\def\csname r@oracle.no_lm.top8\endcsname{55.49}
\expandafter\def\csname r@oracle.top1.beam128\endcsname{47.63}
\expandafter\def\csname r@oracle.top128.all\endcsname{45.10}
\expandafter\def\csname r@oracle.top128.src.coh\endcsname{55.00}
\expandafter\def\csname r@oracle.top128.src.dg\endcsname{34.97}
\expandafter\def\csname r@oracle.top128.src.edited\endcsname{49.27}
\expandafter\def\csname r@oracle.union\endcsname{44.92}
\expandafter\def\csname r@price.better.max\endcsname{0.96}
\expandafter\def\csname r@price.better.min\endcsname{0.10}
\expandafter\def\csname r@ref.audio\endcsname{1673}
\expandafter\def\csname r@ref.cohere_b1\endcsname{15}
\expandafter\def\csname r@ref.cohere_b16\endcsname{80}
\expandafter\def\csname r@ref.ctc_b1\endcsname{174}
\expandafter\def\csname r@ref.ctc_b16\endcsname{141}
\expandafter\def\csname r@ref.ctclm\endcsname{136}
\expandafter\def\csname r@ref.joint_orig\endcsname{1.7}
\expandafter\def\csname r@ref.mem_cohere\endcsname{6.4}
\expandafter\def\csname r@ref.mem_ctc\endcsname{3.8}
\expandafter\def\csname r@ref.mem_nemo\endcsname{8.3}
\expandafter\def\csname r@ref.nemo_b1\endcsname{131}
\expandafter\def\csname r@ref.nemo_b16\endcsname{183}
\expandafter\def\csname r@res.cohere.casablanca_uae.clean16k.cer\endcsname{20.35}
\expandafter\def\csname r@res.cohere.casablanca_uae.clean16k.wer\endcsname{48.35}
\expandafter\def\csname r@res.cohere.casablanca_uae.tel8k.cer\endcsname{24.38}
\expandafter\def\csname r@res.cohere.casablanca_uae.tel8k.wer\endcsname{53.15}
\expandafter\def\csname r@res.cohere.nexdata_cs_sample.clean16k.cer\endcsname{10.05}
\expandafter\def\csname r@res.cohere.nexdata_cs_sample.clean16k.wer\endcsname{19.27}
\expandafter\def\csname r@res.cohere.nexdata_cs_sample.tel8k.cer\endcsname{10.92}
\expandafter\def\csname r@res.cohere.nexdata_cs_sample.tel8k.wer\endcsname{20.53}
\expandafter\def\csname r@res.cohere.sauditalk_longform.clean16k.cer\endcsname{29.51}
\expandafter\def\csname r@res.cohere.sauditalk_longform.clean16k.wer\endcsname{56.75}
\expandafter\def\csname r@res.cohere.sauditalk_longform.tel8k.cer\endcsname{28.40}
\expandafter\def\csname r@res.cohere.sauditalk_longform.tel8k.wer\endcsname{55.80}
\expandafter\def\csname r@res.n.casablanca_uae\endcsname{813}
\expandafter\def\csname r@res.n.nexdata_cs_sample\endcsname{48}
\expandafter\def\csname r@res.n.sauditalk_longform\endcsname{133}
\expandafter\def\csname r@res.nemo.casablanca_uae.clean16k.cer\endcsname{17.09}
\expandafter\def\csname r@res.nemo.casablanca_uae.clean16k.wer\endcsname{53.27}
\expandafter\def\csname r@res.nemo.casablanca_uae.tel8k.cer\endcsname{19.81}
\expandafter\def\csname r@res.nemo.casablanca_uae.tel8k.wer\endcsname{56.56}
\expandafter\def\csname r@res.nemo.nexdata_cs_sample.clean16k.cer\endcsname{8.58}
\expandafter\def\csname r@res.nemo.nexdata_cs_sample.clean16k.wer\endcsname{24.12}
\expandafter\def\csname r@res.nemo.nexdata_cs_sample.tel8k.cer\endcsname{9.85}
\expandafter\def\csname r@res.nemo.nexdata_cs_sample.tel8k.wer\endcsname{25.41}
\expandafter\def\csname r@res.nemo.sauditalk_longform.clean16k.cer\endcsname{25.76}
\expandafter\def\csname r@res.nemo.sauditalk_longform.clean16k.wer\endcsname{61.25}
\expandafter\def\csname r@res.nemo.sauditalk_longform.tel8k.cer\endcsname{27.22}
\expandafter\def\csname r@res.nemo.sauditalk_longform.tel8k.wer\endcsname{62.63}
\expandafter\def\csname r@res.v3_tel.casablanca_uae.clean16k.greedy.cer\endcsname{19.93}
\expandafter\def\csname r@res.v3_tel.casablanca_uae.clean16k.greedy.wer\endcsname{62.79}
\expandafter\def\csname r@res.v3_tel.casablanca_uae.clean16k.lm.cer\endcsname{21.26}
\expandafter\def\csname r@res.v3_tel.casablanca_uae.clean16k.lm.wer\endcsname{54.63}
\expandafter\def\csname r@res.v3_tel.casablanca_uae.tel8k.greedy.cer\endcsname{23.36}
\expandafter\def\csname r@res.v3_tel.casablanca_uae.tel8k.greedy.wer\endcsname{67.24}
\expandafter\def\csname r@res.v3_tel.casablanca_uae.tel8k.lm.cer\endcsname{25.38}
\expandafter\def\csname r@res.v3_tel.casablanca_uae.tel8k.lm.wer\endcsname{58.82}
\expandafter\def\csname r@res.v3_tel.nexdata_cs_sample.clean16k.greedy.cer\endcsname{11.07}
\expandafter\def\csname r@res.v3_tel.nexdata_cs_sample.clean16k.greedy.wer\endcsname{34.50}
\expandafter\def\csname r@res.v3_tel.nexdata_cs_sample.clean16k.lm.cer\endcsname{11.91}
\expandafter\def\csname r@res.v3_tel.nexdata_cs_sample.clean16k.lm.wer\endcsname{29.62}
\expandafter\def\csname r@res.v3_tel.nexdata_cs_sample.tel8k.greedy.cer\endcsname{12.13}
\expandafter\def\csname r@res.v3_tel.nexdata_cs_sample.tel8k.greedy.wer\endcsname{37.04}
\expandafter\def\csname r@res.v3_tel.nexdata_cs_sample.tel8k.lm.cer\endcsname{12.72}
\expandafter\def\csname r@res.v3_tel.nexdata_cs_sample.tel8k.lm.wer\endcsname{30.63}
\expandafter\def\csname r@res.v3_tel.sauditalk_longform.clean16k.greedy.cer\endcsname{28.61}
\expandafter\def\csname r@res.v3_tel.sauditalk_longform.clean16k.greedy.wer\endcsname{70.17}
\expandafter\def\csname r@res.v3_tel.sauditalk_longform.clean16k.lm.cer\endcsname{29.60}
\expandafter\def\csname r@res.v3_tel.sauditalk_longform.clean16k.lm.wer\endcsname{65.29}
\expandafter\def\csname r@res.v3_tel.sauditalk_longform.tel8k.greedy.cer\endcsname{30.47}
\expandafter\def\csname r@res.v3_tel.sauditalk_longform.tel8k.greedy.wer\endcsname{72.46}
\expandafter\def\csname r@res.v3_tel.sauditalk_longform.tel8k.lm.cer\endcsname{31.36}
\expandafter\def\csname r@res.v3_tel.sauditalk_longform.tel8k.lm.wer\endcsname{66.56}
\expandafter\def\csname r@res.v3_wide.casablanca_uae.clean16k.greedy.cer\endcsname{19.90}
\expandafter\def\csname r@res.v3_wide.casablanca_uae.clean16k.greedy.wer\endcsname{62.64}
\expandafter\def\csname r@res.v3_wide.casablanca_uae.clean16k.lm.cer\endcsname{21.78}
\expandafter\def\csname r@res.v3_wide.casablanca_uae.clean16k.lm.wer\endcsname{55.03}
\expandafter\def\csname r@res.v3_wide.casablanca_uae.tel8k.greedy.cer\endcsname{24.14}
\expandafter\def\csname r@res.v3_wide.casablanca_uae.tel8k.greedy.wer\endcsname{68.07}
\expandafter\def\csname r@res.v3_wide.casablanca_uae.tel8k.lm.cer\endcsname{26.60}
\expandafter\def\csname r@res.v3_wide.casablanca_uae.tel8k.lm.wer\endcsname{59.56}
\expandafter\def\csname r@res.v3_wide.nexdata_cs_sample.clean16k.greedy.cer\endcsname{11.00}
\expandafter\def\csname r@res.v3_wide.nexdata_cs_sample.clean16k.greedy.wer\endcsname{35.57}
\expandafter\def\csname r@res.v3_wide.nexdata_cs_sample.clean16k.lm.cer\endcsname{11.68}
\expandafter\def\csname r@res.v3_wide.nexdata_cs_sample.clean16k.lm.wer\endcsname{30.33}
\expandafter\def\csname r@res.v3_wide.nexdata_cs_sample.tel8k.greedy.cer\endcsname{12.30}
\expandafter\def\csname r@res.v3_wide.nexdata_cs_sample.tel8k.greedy.wer\endcsname{39.79}
\expandafter\def\csname r@res.v3_wide.nexdata_cs_sample.tel8k.lm.cer\endcsname{12.80}
\expandafter\def\csname r@res.v3_wide.nexdata_cs_sample.tel8k.lm.wer\endcsname{31.10}
\expandafter\def\csname r@res.v3_wide.sauditalk_longform.clean16k.greedy.cer\endcsname{28.56}
\expandafter\def\csname r@res.v3_wide.sauditalk_longform.clean16k.greedy.wer\endcsname{69.78}
\expandafter\def\csname r@res.v3_wide.sauditalk_longform.clean16k.lm.cer\endcsname{29.77}
\expandafter\def\csname r@res.v3_wide.sauditalk_longform.clean16k.lm.wer\endcsname{64.81}
\expandafter\def\csname r@res.v3_wide.sauditalk_longform.tel8k.greedy.cer\endcsname{31.08}
\expandafter\def\csname r@res.v3_wide.sauditalk_longform.tel8k.greedy.wer\endcsname{72.52}
\expandafter\def\csname r@res.v3_wide.sauditalk_longform.tel8k.lm.cer\endcsname{32.60}
\expandafter\def\csname r@res.v3_wide.sauditalk_longform.tel8k.lm.wer\endcsname{66.84}
\expandafter\def\csname r@sada.cohere.clean16k.cer\endcsname{27.59}
\expandafter\def\csname r@sada.cohere.clean16k.wer\endcsname{46.85}
\expandafter\def\csname r@sada.cohere.tel8k.cer\endcsname{29.00}
\expandafter\def\csname r@sada.cohere.tel8k.wer\endcsname{47.88}
\expandafter\def\csname r@sada.h.train\endcsname{121.6}
\expandafter\def\csname r@sada.n.test\endcsname{4,971}
\expandafter\def\csname r@sada.n.train\endcsname{77,514}
\expandafter\def\csname r@sada.nemo.clean16k.cer\endcsname{21.21}
\expandafter\def\csname r@sada.nemo.clean16k.wer\endcsname{46.50}
\expandafter\def\csname r@sada.nemo.tel8k.cer\endcsname{22.62}
\expandafter\def\csname r@sada.nemo.tel8k.wer\endcsname{48.22}
\expandafter\def\csname r@sada.tel_vs_wide.clean\endcsname{0.19}
\expandafter\def\csname r@sada.tel_vs_wide.tel\endcsname{0.67}
\expandafter\def\csname r@sada.v2.sada_test_clean16k.greedy.cer\endcsname{31.87}
\expandafter\def\csname r@sada.v2.sada_test_clean16k.greedy.wer\endcsname{71.06}
\expandafter\def\csname r@sada.v2.sada_test_clean16k.lm.cer\endcsname{32.44}
\expandafter\def\csname r@sada.v2.sada_test_clean16k.lm.wer\endcsname{59.84}
\expandafter\def\csname r@sada.v2.sada_test_tel8k.greedy.cer\endcsname{35.28}
\expandafter\def\csname r@sada.v2.sada_test_tel8k.greedy.wer\endcsname{74.16}
\expandafter\def\csname r@sada.v2.sada_test_tel8k.lm.cer\endcsname{36.12}
\expandafter\def\csname r@sada.v2.sada_test_tel8k.lm.wer\endcsname{63.55}
\expandafter\def\csname r@sada.v3_tel.sada_test_clean16k.greedy.cer\endcsname{25.05}
\expandafter\def\csname r@sada.v3_tel.sada_test_clean16k.greedy.wer\endcsname{59.98}
\expandafter\def\csname r@sada.v3_tel.sada_test_clean16k.lm.cer\endcsname{24.16}
\expandafter\def\csname r@sada.v3_tel.sada_test_clean16k.lm.wer\endcsname{48.55}
\expandafter\def\csname r@sada.v3_tel.sada_test_tel8k.greedy.cer\endcsname{27.38}
\expandafter\def\csname r@sada.v3_tel.sada_test_tel8k.greedy.wer\endcsname{63.33}
\expandafter\def\csname r@sada.v3_tel.sada_test_tel8k.lm.cer\endcsname{26.85}
\expandafter\def\csname r@sada.v3_tel.sada_test_tel8k.lm.wer\endcsname{51.58}
\expandafter\def\csname r@sada.v3_wide.sada_test_clean16k.greedy.cer\endcsname{25.29}
\expandafter\def\csname r@sada.v3_wide.sada_test_clean16k.greedy.wer\endcsname{60.06}
\expandafter\def\csname r@sada.v3_wide.sada_test_clean16k.lm.cer\endcsname{24.41}
\expandafter\def\csname r@sada.v3_wide.sada_test_clean16k.lm.wer\endcsname{48.36}
\expandafter\def\csname r@sada.v3_wide.sada_test_tel8k.greedy.cer\endcsname{28.35}
\expandafter\def\csname r@sada.v3_wide.sada_test_tel8k.greedy.wer\endcsname{63.45}
\expandafter\def\csname r@sada.v3_wide.sada_test_tel8k.lm.cer\endcsname{28.15}
\expandafter\def\csname r@sada.v3_wide.sada_test_tel8k.lm.wer\endcsname{52.25}
\expandafter\def\csname r@speed.cohere.cpu_rtfx\endcsname{9.20}
\expandafter\def\csname r@speed.cohere.gpu_mem\endcsname{4.76}
\expandafter\def\csname r@speed.cohere.gpu_rtfx16\endcsname{157}
\expandafter\def\csname r@speed.cohere.gpu_rtfx32\endcsname{222}
\expandafter\def\csname r@speed.cpu.audio_min\endcsname{13}
\expandafter\def\csname r@speed.eg2.cpu_rtfx\endcsname{31.10}
\expandafter\def\csname r@speed.eg2.enc_rtfx\endcsname{348}
\expandafter\def\csname r@speed.eg2.gpu_mem\endcsname{1.49}
\expandafter\def\csname r@speed.eg2.gpu_rtfx\endcsname{257}
\expandafter\def\csname r@speed.gpu.audio_min\endcsname{56}
\expandafter\def\csname r@speed.lm.corehours\endcsname{12}
\expandafter\def\csname r@speed.lm.cpu1_rtfx\endcsname{84}
\expandafter\def\csname r@speed.nemo.cpu_rtfx\endcsname{22.60}
\expandafter\def\csname r@speed.nemo.cpu_rtfx_beam\endcsname{19.40}
\expandafter\def\csname r@speed.ratio.cpu\endcsname{3.4}
\expandafter\def\csname r@speed.ratio.cpu_nemo\endcsname{1.4}
\expandafter\def\csname r@speed.ratio.gpu16\endcsname{1.6}
\expandafter\def\csname r@speed.ratio.mem\endcsname{3.2}
\makeatother
\newcommand{\R}[1]{\ifcsname r@#1\endcsname\csname r@#1\endcsname\else\textbf{??#1}\fi}

